Revisiting Discrete Soft Actor-Critic

We study the adaption of Soft Actor-Critic (SAC), which is considered as a state-of-the-art reinforcement learning (RL) algorithm, from continuous action space to discrete action space. We revisit vanilla discrete SAC and provide an in-depth understanding of its Q value underestimation and performance instability issues when applied to discrete settings. We thereby propose Stable Discrete SAC (SDSAC), an algorithm that leverages entropy-penalty and double average Q-learning with Q-clip to address these issues. Extensive experiments on typical benchmarks with discrete action space, including Atari games and a large-scale MOBA game, show the efficacy of our proposed method. Our code is at: https://github.com/coldsummerday/SD-SAC.git.

==> body/introduction.tex <==


\section{Introduction}
Model-free deep reinforcement learning (RL) algorithms have been applied in a range of challenging domains, including games, robotic control and designing chip placement. In the model-free RL paradigm, an agent can be trained by learning an approximator of action-value (Q) function. The class of actor-critic algorithms evaluates the policy function by approximating the value function. Motivated by the maximum-entropy RL, Soft Actor-Critic (SAC) introduces action entropy in the framework of actor-critic to achieve exploit-explore trade-off. SAC has achieved remarkable performance on a range of environments with continuous action spaces.

Soft Actor-Critic\cite{haarnoja2018sacv1,haarnoja2018sacapps} is an off-policy actor-critic reinforcement learning algorithm and it has achieved remarkable performance on a range of continuous-control benchmark tasks. However, many tasks of interest, most notably atari games and chess tasks, have discrete action spaces. Extending SAC with maximum entropy reinforcement learning to discrete actions to accommodate more domains still lacks an accepted practice. Simple discretization of the continuous action output and q-value in a vanilla SAC is an obvious strategy suggested by \cite{christodoulou2019sacd} to adapt SAC to discrete domains named discrete SAC, however this approach had not been as successful as SAC in discrete action spaces.

It is worthwhile to investigate the causes of the performance discrepancy between continuous and discrete domains with SAC. A preliminary understanding is that unreasonable setting of target-entropy for temperature alpha broken the SAC value–entropy trade-off\cite{wang2020metasac,xu2021targetannealing}. Additionally, compared to optimizing parameters of gaussian distribution as policy in continuous SAC, directly optimizing action probability in discrete SAC makes optimize objective of deterministic policy and maximum entropy mutual coupling and worsened the instability Furthermore, function approximation errors of q value are known to lead to estimation bias and hurt performance. Following clipped double q-learning for actor-critic\cite{fujimoto2018td3}, discrete SAC avoids overestimation bias. However, using the lower bound approximation to the critic leads to an underestimation bias\cite{ciosek2019oac,pan2020softmax}, which makes policy fall into pessimistic underexplore.

To address aforementioned issues, we revisit vanilla discrete sac on estimating q-value and optimize objective. Intuitively, a sudden change in policy causes a shift in the entropy, which creates a fast shifting target for the critic network training process due to soft value-learning objective. In contrast, the critic network in SAC takes time to adapt oscillating target process and exacerbates policy instability. We point out potential issue that lacking  constraints for trust region policy update with current optimize objective in discrete SAC. We suggested an extra entropy penalty on the policy optimize objective to constraint policy update which ensure the stability of discrete sac training process. On the other hand, previous works\cite{fujimoto2018td3,duan2021distributionalsac} focused on overestimate bias on q-function-based methods, however, we observed underestimate bias phenomenon in discrete SAC. Discrete SAC enters pessimistic exploration when when reward become sparse. We propose alternative design choice as double average q-learning and q-approximation-clip to limit q-value within a suitable range.

In this paper, we design simple test cases to isolate two failure modes where vanilla SAC does not achieve the desired convergence behavior in discrete action space. Correspondingly, we propose two alternative design choices as policy-penalty and double average q-learning with q-approximation-clip to solve the above dilemma.Given the recent concerns in reproducibility\cite{henderson2018matters}, we run our experiments across multiple seeds with fair evaluation metrics. Not only did we verify our contributions on atari games, but we deployed it to the Honor of kings 1V1, a large-scale MOBA mobile game, to demonstrate the scale-up capacity of sac-discrete with our contribution.

To sum up, the key contributions of this paper are featured as follows:
\begin{enumerate}

    \item  Policy instability with discrete sac on training process due to lacking constraints for trust region policy update. We propose entropy-penalty to improve unstable performance of discrete sac.
    \item We pay attention to the underestimation bias of discrete sac and analyze the negative impact for pessimistic underexplore caused by underestimation bias. To Address this issue, double average q-learning with q-approximation-clip is suggested to estimate state-action value.
    \item We offer an empirical evaluation of our alternative design decisions for both atari games and large-scale MOBA game Honor of kings 1V1.

 \end{enumerate}

The remaining contents of this paper are organized as follows. SAC background and related works are overviewed in Section II. Analysis of failure modes of vanilla discrete SAC are presented in Section III. We present improvements for SAC failure modes and experimental results in Section IV. The paper ends in Section V with discussion.



==> body/introduction_0821.tex <==


\section{Introduction}
Soft Actor-Critic\cite{haarnoja2018sacv1,haarnoja2018sacapps} is an off-policy actor-critic reinforcement learning algorithm and it has achieved remarkable performance on a range of continuous-control benchmark tasks. However, many tasks of interest, most notably atari games and chess tasks, have discrete action spaces. Extending SAC with maximum entropy reinforcement learning to discrete actions to accommodate more domains still lacks an accepted practice. Simple discretization of the continuous action output and q-value in a vanilla SAC is an obvious strategy suggested by \cite{christodoulou2019sacd} to adapt SAC to discrete domains named discrete SAC, however this approach had not been as successful as SAC in discrete action spaces.

It is worthwhile to investigate the causes of the performance discrepancy between continuous and discrete domains with SAC. A preliminary understanding is that unreasonable setting of target-entropy for temperature alpha broken the SAC value–entropy trade-off\cite{wang2020metasac,xu2021targetannealing}. Additionally, compared to optimizing parameters of gaussian distribution as policy in continuous SAC, directly optimizing action probability in discrete SAC makes optimize objective of deterministic policy and maximum entropy mutual coupling and worsened the instability Furthermore, function approximation errors of q value are known to lead to estimation bias and hurt performance. Following clipped double q-learning for actor-critic\cite{fujimoto2018td3}, discrete SAC avoids overestimation bias. However, using the lower bound approximation to the critic leads to an underestimation bias\cite{ciosek2019oac,pan2020softmax}, which makes policy fall into pessimistic underexplore.

To address aforementioned issues, we revisit vanilla discrete sac on estimating q-value and optimize objective. Intuitively, a sudden change in policy causes a shift in the entropy, which creates a fast shifting target for the critic network training process due to soft value-learning objective. In contrast, the critic network in SAC takes time to adapt oscillating target process and exacerbates policy instability. We point out potential issue that lacking  constraints for trust region policy update with current optimize objective in discrete SAC. We suggested an extra entropy penalty on the policy optimize objective to constraint policy update which ensure the stability of discrete sac training process. On the other hand, previous works\cite{fujimoto2018td3,duan2021distributionalsac} focused on overestimate bias on q-function-based methods, however, we observed underestimate bias phenomenon in discrete SAC. Discrete SAC enters pessimistic exploration when when reward become sparse. We propose alternative design choice as double average q-learning and q-approximation-clip to limit q-value within a suitable range.

In this paper, we design simple test cases to isolate two failure modes where vanilla SAC does not achieve the desired convergence behavior in discrete action space. Correspondingly, we propose two alternative design choices as policy-penalty and double average q-learning with q-approximation-clip to solve the above dilemma.Given the recent concerns in reproducibility\cite{henderson2018matters}, we run our experiments across multiple seeds with fair evaluation metrics. Not only did we verify our contributions on atari games, but we deployed it to the Honor of kings 1V1, a large-scale MOBA mobile game, to demonstrate the scale-up capacity of sac-discrete with our contribution.

To sum up, the key contributions of this paper are featured as follows:
\begin{enumerate}

    \item  Policy instability with discrete sac on training process due to lacking constraints for trust region policy update. We propose entropy-penalty to improve unstable performance of discrete sac.
    \item We pay attention to the underestimation bias of discrete sac and analyze the negative impact for pessimistic underexplore caused by underestimation bias. To Address this issue, double average q-learning with q-approximation-clip is suggested to estimate state-action value.
    \item We offer an empirical evaluation of our alternative design decisions for both atari games and large-scale MOBA game Honor of kings 1V1.

 \end{enumerate}

The remaining contents of this paper are organized as follows. SAC background and related works are overviewed in Section II. Analysis of failure modes of vanilla discrete SAC are presented in Section III. We present improvements for SAC failure modes and experimental results in Section IV. The paper ends in Section V with discussion.



==> body/test_eqution.tex <==
% \section{test}
% \begin{figure*} [t!]
% 	\subfloat[baseline discrete sac]{
% 		\includegraphics[width=0.23\textwidth]{images/experiments/loss_surfaces/base_loss_surface_show.png}
% 		}
% 	\subfloat[our method]{
% 		\includegraphics[width=0.23\textwidth]{images/experiments/loss_surfaces/total_loss_surface_show.png}
% 		}

% 	\caption{1dfkjsdjfsdfks}
% 	\label{fig3} 
% \end{figure*}

% \cite{sub_fig_1}

$$
V_{true} = r + [Q(s,a)-\alpha \log (\pi(a \mid s)] 
$$
$$
V_{appox} = r + \min _{i=1,2}[(Q_{\theta_{i}}(s,a)+\epsilon ) -\alpha \log (\pi(a \mid s)]
$$
% \end{equation*}

$\epsilon$
